Asymmetric Forward-Backward-Adjoint Splitting for Solving Monotone Inclusions Involving Three Operators

In this work we propose a new splitting technique, namely Asymmetric Forward-Backward-Adjoint splitting, for solving monotone inclusions involving three terms, a maximally monotone, a cocoercive and a bounded linear operator. Classical operator splitting methods, like Douglas-Rachford and Forward-Backward splitting are special cases of our new algorithm. Asymmetric Forward-Backward-Adjoint splitting unifies, extends and sheds light on the connections between many seemingly unrelated primal-dual algorithms for solving structured convex optimization problems proposed in recent years. More importantly, it greatly extends the scope and applicability of splitting techniques to a wider variety of problems. One important special case leads to a Douglas-Rachford type scheme that includes a third cocoercive operator.

==> section-4.tex <==
\section{{Convergence Analysis}} \label{sec:4}
In this section we present the main theorem of the paper that analyzes the convergence of \Cref{Algorithm-1}. 
\begin{thm} 
\begin{singlespace}
\label{thm:Suppose-that-} Consider \Cref{Algorithm-1} with $\Sigma=\zer(A+M+C)\neq\textrm{Ø}$.
Let \Cref{enu:-is-maximally,enu:Let--and} hold.
Suppose $(\lambda_{n})_{n\in\Nn}$ is a sequence in $]0,\delta[$,
with 
\begin{equation}
\delta=2-\frac{1}{2\beta},\quad\delta>0,\quad\sum_{n\in\Nn}\lambda_{n}(\delta-\lambda_{n})=+\infty\label{eq:-7}
\end{equation}
Then,
\begin{enumerate}[{label=(\textit{\roman*})},ref=\textit{\roman{*}}]

\item \label{thm-part1} $(z_{n})_{n\in\Nn}$ is F\'{e}jer monotone with respect to $\Sigma$ in the Hilbert space $\HH_{S}$.
\item \label{thm-part2}$(\tilde{z}_{n})_{n\in\Nn}$ converges strongly to zero.
\item $(z_{n})_{n\in\Nn}$ converges weakly to a point in $\Sigma$.
\item Let $\lambda_{n}$ be uniformly bounded between 0 and $\delta$. If there exists $\nu>0$ and $\eta>0$ such that 
\begin{equation}
d(z,\Sigma)\leq\eta\|w\|\;\;\forall z\;and\;w\in(A+M+C)z\;when\;\|w\|\leq\nu\label{eq:-38}
\end{equation}
then the convergence is $Q$-linear.\footnote{The sequence ${x_{n}}$ converges to $x^{\star}$ $Q$-linearly with $Q$-factor given by $\sigma\in]0,1[$, if for $n$ sufficiently large  $\|x_{n+1}-x^{\star}\|\leq\sigma\|x_{n}-x^{\star}\|$ holds.}
\end{enumerate}
	Furthermore, when the cocoercive term $C$ is absent all of the above statements hold with $\delta=2$. 
	\end{singlespace}
\end{thm}
\begin{proof}
The operators $\tilde{A}=P^{-1}(A+K)$ and $\tilde{B}=P^{-1}(M+C-K)$
are monotone in the Hilbert space $\HH_{P}$. We observe that
\[
\bar{z}_{n}=[H+A]^{-1}[H-M-C]z_{n}=[I+\tilde{A}]^{-1}[I-\tilde{B}]z_{n}
\]
Therefore $z_{n}-\tilde{B}z_{n}\in\bar{z}_{n}+\tilde{A}\bar{z}_{n}$,
or $-\tilde{z}_{n}-\tilde{B}z_{n}\in\tilde{A}\bar{z}_{n}$. Since $-\tilde{B}z^{\star}\in\tilde{A}z^{\star}$
for $z^{\star}\in\zer(A+M+C)$ by monotonicity of $\tilde{A}$ on $\HH_{P}$ we have
\begin{align}
\langle\tilde{B}z_{n}-\tilde{B}z^{\star}+\tilde{z}_{n},z^{\star}-\bar{z}_{n}\rangle_{P} \geq0. \nonumber
\end{align}
Then, 
\begin{align}
0 & \leq\langle\tilde{B}z_{n}-\tilde{B}z^{\star}+\tilde{z}_{n},z^{\star}-\bar{z}_{n}\rangle_{P}\nonumber \\
 & =\langle P^{-1}(M-K)(z_{n}-z^{\star})+P^{-1}(Cz_{n}-Cz^{\star})+\tilde{z}_{n},z^{\star}-\bar{z}_{n}\rangle_{P}\nonumber \\
 & =\langle(M-K)(z_{n}-z^{\star})+Cz_{n}-Cz^{\star}+P\tilde{z}_{n},z^{\star}-\bar{z}_{n}\rangle.\label{eq:-3-2}
\end{align}
On the other hand
\begin{align*}
\langle Cz_{n}-Cz^{\star},z^{\star}-\bar{z}_{n}\rangle & =\langle Cz_{n}-Cz^{\star},z_{n}-\bar{z}_{n}\rangle+\langle Cz_{n}-Cz^{\star},z^{\star}-z_{n}\rangle\\
 & \leq\frac{\epsilon}{2}\|\tilde{z}_{n}\|_{P}^{2}+\frac{1}{2\epsilon}\|Cz_{n}-Cz^{\star}\|_{P^{-1}}^{2}+\langle Cz_{n}-Cz^{\star},z^{\star}-z_{n}\rangle\\
 & \leq\frac{\epsilon}{2}\|\tilde{z}_{n}\|_{P}^{2}+(1-\frac{1}{2\epsilon\beta})\langle Cz_{n}-Cz^{\star},z^{\star}-z_{n}\rangle.
\end{align*}
The second inequality follows from Young-Fenchel's inequality with
parameter $\epsilon>0$ and the third inequality follows from $\beta$-cocoercivity
of $C$ with respect to the $P$ norm. Set $\epsilon\coloneqq\frac{1}{2\beta}$ so that
\begin{align}
\langle Cz_{n}-Cz^{\star},z^{\star}-\bar{z}_{n}\rangle & \leq\frac{1}{4\beta}\|\tilde{z}_{n}\|_{P}^{2}.\label{eq:-4-2}
\end{align}
In turn, \eqref{eq:-3-2}, \eqref{eq:-4-2} and monotonicity of $M-K$,
yield
\begin{align*}
0 & \leq\langle(M-K)(z_{n}-z^{\star})+Cz_{n}-Cz^{\star}+P\tilde{z}_{n},z^{\star}-\bar{z}_{n}\rangle\\
 & =\langle(M-K)(z_{n}-z^{\star}),z^{\star}-z_{n}\rangle+\langle(M-K)(z_{n}-z^{\star}),z_{n}-\bar{z}_{n}\rangle\\
 & +\frac{1}{4\beta}\|\tilde{z}_{n}\|_{P}^{2}+\langle P\tilde{z}_{n},z^{\star}-z_{n}\rangle+\langle P\tilde{z}_{n},z_{n}-\bar{z}_{n}\rangle\\
 & \leq\langle z_{n}-z^{\star},(M^{*}+K)(z_{n}-\bar{z}_{n})\rangle\\
 & +\frac{1}{4\beta}\|\tilde{z}_{n}\|_{P}^{2}+\langle P\tilde{z}_{n},z^{\star}-z_{n}\rangle-\|\tilde{z}_{n}\|_{P}^{2}\\
 & =\langle z_{n}-z^{\star},-(M^{*}+H)\tilde{z}_{n}\rangle-(1-\frac{1}{4\beta})\|\tilde{z}_{n}\|_{P}^{2}.
\end{align*}
We have 
\begin{equation}
\langle z_{n}-z^{\star},(M^{*}+H)\tilde{z}_{n}\rangle\leq-(1-\frac{1}{4\beta})\|\tilde{z}_{n}\|_{P}^{2}. \label{eq:42-42-11}
\end{equation}
For notation convenience define $\delta\coloneqq2-\frac{1}{2\beta}$. We show that $\|z_{n}-z^{\star}\|_S$ is decreasing using \eqref{eq:42-42-11} together with \hyperlink{alg:line3}{line 3} and \hyperlink{alg:line3}{4} of \Cref{Algorithm-1}:
\begin{align}
\|z_{n+1}-z^{\star}\|_{S}^{2} & =\|z_{n}-z^{\star}+\alpha_{n}S^{-1}(H+M^{*})\tilde{z}_{n}\|_{S}^{2} \nonumber \\
 & =\|z_{n}-z^{\star}\|_{S}^{2}+2\alpha_{n}\langle z_{n}-z^{\star},(H+M^{*})\tilde{z}_{n}\rangle+\alpha_{n}^{2}\|S^{-1/2}(H+M^{*})\tilde{z}_{n}\|^{2} \nonumber \\
 & \leq\|z_{n}-z^{\star}\|_{S}^{2}-\alpha_{n}\delta\|\tilde{z}_{n}\|_{P}^{2}+\alpha_{n}^{2}\|S^{-1/2}(H+M^{*})\tilde{z}_{n}\|^{2}\nonumber \\
 & =\|z_{n}-z^{\star}\|_{S}^{2}-\delta\lambda_{n}\frac{\|\tilde{z}_{n}\|_{P}^{4}}{\|S^{-1/2}(H+M^{*})\tilde{z}_{n}\|^{2}}+\lambda_{n}^{2}\frac{\|\tilde{z}_{n}\|_{P}^{4}}{\|S^{-1/2}(H+M^{*})\tilde{z}_{n}\|^{2}}\nonumber \\
 & =\|z_{n}-z^{\star}\|_{S}^{2}-\lambda_{n}(\delta-\lambda_{n})\|S^{-1/2}\left(H+M^{*}\right)\tilde{z}_{n}\|^{-2}\|\tilde{z}_{n}\|_{P}^{4}\nonumber \\
 & =\|z_{n}-z^{\star}\|_{S}^{2}-\lambda_{n}(\delta-\lambda_{n})\|P^{-1/2}S^{-1/2}\left(H+M^{*}\right)\tilde{z}_{n}\|_{P}^{-2}\|\tilde{z}_{n}\|_{P}^{4}\nonumber \\
 & \leq\|z_{n}-z^{\star}\|_{S}^{2}-\lambda_{n}(\delta-\lambda_{n})\|P^{-1/2}S^{-1/2}\left(H+M^{*}\right)\|_{P}^{-2}\|\tilde{z}_{n}\|_{P}^{2}\nonumber \\
 & =\|z_{n}-z^{\star}\|_{S}^{2}-\lambda_{n}(\delta-\lambda_{n})\|S^{-1/2}\left(H+M^{*}\right)P^{-1/2}\|^{-2}\|\tilde{z}_{n}\|_{P}^{2}. \label{eq:-12-23}
\end{align}
When the cocoercive term, $C$, is absent it is straight forward to see that the above inequality holds with $\delta=2$. \\
\textit{(i)}: Inequality \eqref{eq:-12-23} and $\lambda_{n}\in]0,\delta[$ prove that $(z_{n})_{n\in\Nn}$
is F\'{e}jer monotone with respect to $\zer(A+M+C)$ in the Hilbert space $\HH_{S}$. \\
\textit{(ii)}: From \eqref{eq:-12-23}
and $\sum_{n\in\Nn}\lambda_{n}(\delta-\lambda_{n})=+\infty$ with
 $\lambda_{n}\in]0,\delta[$, it follows that $\tilde{z}_{n}\overset{s}{\rightarrow}0$. \\
\textit{(iii)}: Define 
\begin{equation}
w_{n}\coloneqq -(H-M-C)\tilde{z}_{n}.\label{eq:-2}
\end{equation}
It follows from \eqref{eq:-2}, \eqref{thm-part2} and cocoercivity of $C$ that
\begin{equation}
w_{n}\overset{s}{\rightarrow}0\label{eq:-4}
\end{equation}
By \hyperlink{alg:line1}{line 1} of \Cref{Algorithm-1} we have $(H-M-C)z_n\in H\bar{z}_n+A\bar{z}_n $, which together with \eqref{eq:-2} yields
\begin{equation}
w_{n}\in A\bar{z}_{n}+M\bar{z}_{n} + C\bar{z}_{n}.\label{eq:-3}
\end{equation}

Now let $z$ be a weak sequential cluster point of $(z_{n})_{n\in\Nn}$
, say $z_{k_{n}}\overset{w}{\rightarrow}z$. It follows from \eqref{thm-part1} that
$\bar{z}_{k_{n}}\overset{w}{\rightarrow}z$, and from \eqref{eq:-4}
that $w_{k_{n}}\overset{s}{\rightarrow}0$. Altogether, by \eqref{eq:-3}, $(\bar{z}_{k_{n}},w_{k_{n}})_{n\in\Nn}$
lies in $\gra(A+M+C)$. Additionally, by \cite[Example 20.28,20.29 and Corollary 24.4(i)]{bauschke2011convex}, $A+M+C$ is maximally monotone. Then, an appeal to \cite[Proposition
20.33(ii)]{bauschke2011convex} yields $(z,0)\in\gra(A+M+C)$. This together with \eqref{thm-part1} and \cite[Theorem
5.5]{bauschke2011convex} completes the proof. \\
\textit{(iv)}: Consider $w_{n}$ defined in \eqref{eq:-3}. By assumption (\ref{eq:-38})
we have 
\[
d(\bar{z}_{n},\Sigma)\leq\eta\|w_{n}\|\;\;when\;\|w_{n}\|\leq\nu.
\]
Since $w_{n}\overset{s}{\rightarrow}0$, there exists
$\bar{n}$ such that $\|w_{n}\|\leq\nu$ for $n>\bar{n}$ and hence
$d(\bar{z}_{n},\Sigma)\leq\eta\|w_{n}\|$. In addition Lipschitz
continuity of $C$, Triangle inequality and Rayleigh quotient, yield 
\begin{align}
\|w_{n}\| & =\|(H-M-C)\tilde{z}_{n}\|\nonumber \\
 & \leq\|(H-M)(z_{n}-\bar{z}_{n})\|+\|C\bar{z}_{n}-Cz_{n}\|\nonumber \\
 & \leq\|H-M\|\|\tilde{z}_{n}\|+\|P\|^{1/2}\|C\bar{z}_{n}-Cz_{n}\|_{P^{-1}}\nonumber \\
 & \leq(\|H-M\|+\frac{1}{\beta}\|P\|)\|\tilde{z}_{n}\|.\nonumber
\end{align}
Then for $z^{\star}\in\Sigma$ satisfying $\|\bar{z}_{n}-z^{\star}\|=d(\bar{z}_{n},\Sigma)$,
(The minimum is attained since $\Sigma$ is a closed convex set), we can write 
\[
\|\bar{z}_{n}-z^{\star}\|=d(\bar{z}_{n},\Sigma)\leq\xi\eta\|\bar{z}_{n}-z_{n}\|
\]
where $\xi=\|H-M\|+\frac{1}{\beta}\|P\|$.
Another application of Triangle inequality and Rayleigh quotient resutls
in 
\begin{align}
\|z_{n}-z^{\star}\| & \leq  \|\bar{z}_{n}-z^{\star}\|+\|\bar{z}_{n}-z_{n}\|\nonumber \\
 & \leq  (\xi\eta+1)\|P^{-1}\|^{1/2}\|\bar{z}_{n}-z_{n}\|_{P}.\label{eq:-40}
\end{align}
By uniform boundedness of $\lambda_n$ we have that there exists $\lambda_m$ and $\lambda_M$ such that $0<\lambda_m\leq\lambda_n\leq\lambda_M <\delta$. Consequently, \eqref{eq:-12-23} and \eqref{eq:-40}  yield
\[
\|z_{n+1}-z^{\star}\|^{2}\leq\kappa\|z_{n}-z^{\star}\|^{2}
\]
where $\kappa=1-\frac{\lambda_{M}(\delta-\lambda_{m})\|S^{-1/2}\left(H+M^{*}\right)P^{-1/2}\|^{-2}}{(\xi\eta+1)^{2}\|P^{-1}\|}$.
This shows that $\{z_{n}\}$ converges $Q$-linearly to $z^{\star}.$
\end{proof}
\begin{rem}
The condition \eqref{eq:-38} is known as calmness of $(A+M+C)^{-1}$ at 0 for $\zer (A+M+C)$ (see \cite[Equation 9(30)]{rockafellar2009variational}) and it is  equivalent to metric subregularity of the operator $A+M+C$ at $\zer (A+M+C)$ for 0 \cite[Theorem 3H.3]{dontchev2009implicit}. The above two properties are weaker versions of Aubin property and metric
regularity respectively. We refer the reader to \cite[Chapter 9]{rockafellar2009variational} and \cite[Chapter 3]{dontchev2009implicit} for extensive discussion.
\end{rem}
\begin{rem}
\label{rem:P}In the special case when $C\equiv0$, $K=M$, $M$
is skew-adjoint and $S=P$, we can choose $P\in\mathscr{B}(\HH)$ to be a self-adjoint,
positive operator rather than strongly positive operator. The convergence
of the Algorithm in this case can be proven following the same line
of reasoning as \cite[Theorem 3.3]{condat2013primal}. 
\end{rem}
\begin{rem}
When $H=\gamma^{-1} \id$, $S=\id$ and $M=0$,  \Cref{Algorithm-1} simplifies to the classic Forward-Backward splitting. If $\beta$ is the cocoercivity constant of $C$ with respect to the canonical norm $\|\cdot\|$, then $\beta/\gamma$ is the cocoercivity constant with respect to the $P$ norm. The condition \eqref{eq:-7} of \Cref{thm:Suppose-that-} becomes
\begin{equation*}
\lambda_{n}\in]0,\delta[ \quad with \quad \delta=2-\frac{\gamma}{2\beta},\quad\gamma<4\beta,\quad\sum_{n\in\Nn}\lambda_{n}(\delta-\lambda_{n})=+\infty
\end{equation*} 
whereas in the classic Forward-Backward splitting we had the same condition with $\gamma\leq2\beta$ or equivalently $\delta\geq 1$ instead of $\delta>0$  (see \cite[Lemma 4.4]{condat2013primal}).  \\
Furthermore, if operator $C$ is also absent we are left with the classic Proximal Point algorithm. Douglas-Rachford method was shown to be a special case of Proximal Point algorithm in \cite{eckstein1992douglas}.  
\end{rem}
\begin{rem}
In \Cref{Algorithm-1}, When $H=\gamma^{-1} \id$, $S=\id$, $C=0$ and $M$ is skew adjoint, we can enforce $\alpha_n=\gamma$  by choosing $\lambda_n=\frac{\gamma\|(\gamma^{-1} \id +M^{*})\tilde{z}_{n}\|^{2}}{\gamma^{-1}\|\tilde{z}_{n}\|^{2}}$. This satisfies the conditions of \Cref{thm:Suppose-that-} if $\|M\|<\gamma^{-1}$ and \Cref{Algorithm-1} becomes
\begin{align*}
\bar{z}_{n} & =[\id+\gamma A]^{-1}[\id-\gamma M]z_{n}\\
z_{n+1} & =\bar{z}_{n}+\gamma M(z_{n}-\bar{z}_{n}).
\end{align*}  
This is Tseng's Forward-Backward-Forward algorithm \cite{tseng2000modified} when we assume the Lipschitz operator to be the skew adjoint operator $M$. 
\end{rem}

==> section-6.tex <==
\section{Extension of g to several composite functions}

Consider the problem 
\[
\underset{x\in\HH}{\minimize}\ f(x)+h(x)+\sum_{i=1}^{r}(g_{i}\oblong l_{i})(L_{i}x)
\]
 where $f\in\Gamma_{0}(\HH)$, $g\in\Gamma_{0}(\mathcal{G}_{i})$
and $L\in\mathscr{B}(\HH,\mathcal{G}_{i})$. Furthermore, $h:\HH\rightarrow\mathbb{R}$
is convex, differentiable on $\HH$ with $\beta_{h}$-Lipschitz gradient
for some $\beta_{h}\in[0,+\infty[$ and let $l_{i}\in\Gamma_{0}(\mathcal{G}_{i})$
be $\beta_{l_{i}}^{-1}$-strongly convex for some $\beta_{l_{i}}\in[0,+\infty[$ for $i=1,\ldots,r$. The optimality conditions can be
written as 
\begin{equation}
\left\{ \begin{array}{c}
0\in\partial f(x)+\nabla h(x)+\sum_{j=1}^{r}L_{j}^{*}y_{j} \qquad\quad\;\\
0\in\partial g_{i}^{*}(y_{i})+\nabla l_{i}^{*}(y_{i})-L_{i}x \quad i=1,\ldots,r
\end{array}\right. \label{eq:primal-dual-several}
\end{equation}
Let $\mathcal{G}=\mathcal{G}_{1}\oplus\cdots\oplus\mathcal{G}_{r}$ and 
let $\mathcal{K}$ be 
\[
\mathcal{K}=\HH\oplus\mathcal{G}
\]
Define 
\[
\underline{g}:\underline{y}\mapsto\sum_{i=1}^{r}g_{i}(y_{i})
\]
\[
\underline{l}:\underline{y}\mapsto\sum_{i=1}^{r}l_{i}(y_{i})
\]
\[
\underline{L}:x\mapsto(L_{1}x,\ldots,L_{r}x)
\]
where  $\underline{y}=(y_{1},\cdots,y_{r})$. We can write the monotone inclusion problem in the form 
\[
0\in Az+Bz
\]
with $z=(x,\underline{y})$ by defining
\[
A:\mathcal{K}\to2^{\mathcal{K}}:(x,\underline{y})\mapsto(\partial f(x),\partial\underline{g}^{*}(\underline{y}))
\]
\[
M\in\mathscr{B}(\mathcal{K}):(x,\underline{y})\mapsto(\underline{L}^{*}\underline{y},-\underline{L}x)
\]
\[
C:\mathcal{K}\to\mathcal{K}:(x,\underline{y})\mapsto(\nabla h(x),\nabla\underline{l}{}^{*}(\underline{y}))
\]
and $Bz=Mz+Cz$. Furthermore, set
\[
H\in\mathscr{B}(\mathcal{K}):(x,\underline{y})\mapsto(\gamma_{1}^{-1}x,H_{21}(x)+\gamma_{2}^{-1}y_{1},\ldots,H_{r+1,1}(x)+\sum\limits_{j=1}^{r-1}H_{r+1,j+1}(y_{j})+\gamma_{r+1}^{-1}y_{r}).
\]

Let $P$ be the symmetric part of $H$ such that $P\in\mathcal{P}_{\tau}(\mathcal{K})$
for some $\tau\in[0,+\infty[$.  Let $H_{i+1,1}=-\theta L_{i}$ for $i=1,\ldots,r$. Then Algorithm \ref{Algorithm-1}, takes the following form
\begin{algorithm}[H]
    \caption{}
	\label{algorithm-9}
    \begin{algorithmic} 
            \item\textbf{Inputs:} $x_0\in\HH$, $y_0\in\mathcal{G}$
            \For{$n=0,\ldots$} 
                \State $\bar{x}_{n} =\prox_{\gamma_{1}f}(x_{n}-\gamma_{1}\sum_{j=1}^{r}L_{j}^{*}y_{j,n}-\gamma_{1}\nabla h(x_{n}))  $
                \State $\bar{y}_{i,n} =\prox_{\gamma_{i+1}g_{i}^{*}}(y_{i,n}+(1-\theta)\gamma_{i+1}L_{i}x_{n}+\theta\gamma_{i+1} L_{i}\bar{x}_{n}  $
                \State $\qquad \, +\sum_{j=2}^{i}H_{i+1,j}(y_{j-1,n}-\bar{y}_{j-1,n})-\gamma_{i+1}\nabla l_{i}^{*}(y_{i,n}))\quad i=1,\ldots,r$
                \State $\tilde{x}_{n} =\bar{x}_{n}-x_{n},\tilde{y}_{i,n}=\bar{y}_{i,n}-y_{i,n}\quad i=1,\ldots,r  $
                \State $\tilde{z}_{n}=(\tilde{x}_{n},\tilde{\underline{y}}_{n})$
                \State $\displaystyle \alpha_{n} =\frac{\lambda_{n}\|\tilde{z}_{n}\|_{P}^{2}}{\|S^{-1/2}\left(H+M^{*}\right)\tilde{z}_{n}\|^{2}}  $ 
                \State $(x_{n+1},\underline{y}_{n+1}) =(x_{n},\underline{y}_{n})+\alpha_{n}S^{-1}(H+M^{*})\tilde{z}_{n}$
            \EndFor
    \end{algorithmic}
\end{algorithm}
 Define 
\[
\bar{H}_{22}\in\mathscr{B}(\mathcal{G}):\underline{y}\mapsto(\gamma_{2}^{-1}y_{1},H_{32}(y_{1})+\gamma_{3}^{-1}y_{2},\cdot\cdot,\sum\limits_{j=1}^{r-1}H_{r+1,j+1}(y_{j})+\gamma_{r+1}^{-1}y_{r})) 
\]
and let $\bar{P}_{22}$ be the symmetric part of $\bar{H}_{22}$.
Then $H$ and $P$ can be rewritten as
\[
H\in\mathscr{B}(\mathcal{K}):(x,\underline{y})\mapsto(\gamma_{1}^{-1}x,-\theta \underline{L}x+\bar{H}_{22}(\underline{y}))
\]
and 
\begin{equation}
P\in\mathscr{B}(\mathcal{K}):(x,\underline{y})\mapsto(\gamma_{1}^{-1}x-\frac{1}{2}\theta\underline{L}^{*}\underline{y},-\frac{1}{2}\theta\underline{L}x+\bar{P}_{22}(\underline{y}))\label{eq:-32-34}
\end{equation}


\begin{lem}
\label{lem:strongly positive p-2}Let $P$ be as in (\ref{eq:-32-34})
Let $\gamma_{1}>0$ and $\bar{P}_{22}$ be strongly positive such that 
\[
\gamma_{1}^{-1}-\frac{\theta^{2}}{4}\|\underline{L}^{*}\bar{P}_{22}^{-1}\underline{L}\|>0
\]
then $P$ is $\tau$-strongly positive with
\[
\tau=\frac{1}{2}\gamma_{1}^{-1}+\frac{1}{2}\|\bar{P}_{22}^{-1}\|^{-1}-\frac{1}{2}\sqrt{\theta^{2}\|\bar{P}_{22}^{-1}\|^{-1}\|\underline{L}^{*}\bar{P}_{22}^{-1}\underline{L}\|+(\gamma_{1}^{-1}-\\\|\bar{P}_{22}^{-1}\|^{-1})^{2}}.
\]
\end{lem}
\begin{proof}
The proof is analogous to that of Lemma \ref{lem:strongly positive p-1}.
\end{proof}

\begin{prop}
\label{cor:coco-2}Consider $(x_{n},\underline{y}_{n})\in\mathcal{K}$  
defined by Algorithm \ref{algorithm-9}.
Let $\beta_{h}\in]0,+\infty[$ and $\beta_{l_{i}}\in]0,+\infty[$ be the
Lipschitz constant of $\nabla h$ and $\nabla l_{i}^{*}$ respectively for $i=1,\ldots,r$. 
Let 
\[
\tau=\frac{1}{2}\gamma_{1}^{-1}+\frac{1}{2}\|\bar{P}_{22}^{-1}\|^{-1}-\frac{1}{2}\sqrt{\theta^{2}\|\bar{P}_{22}^{-1}\|^{-1}\|\underline{L}^{*}\bar{P}_{22}^{-1}\underline{L}\|+(\gamma_{1}^{-1}-\\\|\bar{P}_{22}^{-1}\|^{-1})^{2}}
\]
and suppose that $(\lambda_{n})_{n\in\Nn}$ is a sequence in $]0,\delta[$,
 with $\delta=2-\frac{1}{2\tau}\max\{\beta_{h},\beta_{l_{1}},\ldots,\beta_{l_{r}}\}$ and $\sum_{n\in\Nn}\lambda_{n}(\delta-\lambda_{n})=+\infty$.
Then if
 \[
 4\tau\min\{\beta_{h}^{-1},\beta_{l_{1}}^{-1},\ldots,\beta_{l_{r}}^{-1}\}>1
 \]
holds, there exists a solution $(x^{\star},\underline{y}^{\star})\in\mathcal{K}$
to the monotone inclusion problem (\ref{eq:primal-dual-several}) such that
$(x_n,\underline{y}_{n})$ converges weakly to $(x^{\star},\underline{y}^{\star})$.
\end{prop}
\begin{proof}
The proof is analogous to the proof of Proposition \ref{cor:coco}.
\end{proof}
\begin{prop}
\label{cor:coco-3}Consider $(x_{n},\underline{y}_{n})\in\mathcal{K}$ defined
by Algorithm \ref{algorithm-9} when $l=\iota_{\{0\}}$. Let $\beta_{h}\in[0,+\infty[$ be the Lipschitz
constant of $\nabla h$. Suppose that $(\lambda_{n})_{n\in\Nn}$ is a sequence in $]0,\delta[$,
 with $\delta=2-\frac{\beta_{h}}{2}(\gamma_{1}^{-1}-\frac{\theta^{2}}{4}\|\underline{L}^{*}\bar{P}_{22}^{-1}\underline{L}\|)^{-1}$ and $\sum_{n\in\Nn}\lambda_{n}(\delta-\lambda_{n})=+\infty$. Then if 
\[
\gamma_{1}^{-1}-\frac{\theta^{2}}{4}\|\underline{L}^{*}\bar{P}_{22}^{-1}\underline{L}\|>\frac{\beta_{h}}{4}
\]
holds, there exists a solution $(x^{\star},\underline{y}^{\star})\in\mathcal{K}$
to the monotone inclusion problem (\ref{eq:primal-dual-several}) such that
$(x_n,\underline{y}_{n})$ converges weakly to $(x^{\star},\underline{y}^{\star})$.
\end{prop}
\begin{proof}
The proof is analogous to the proof of Proposition \ref{cor:coco-1}.
\end{proof}

\subsection{Without Gauss Siedel updates on dual variables}
Consider Algorithm \ref{algorithm-9} and let the other
off diagonal elements to be zero to derive the following algorithm
\begin{algorithm}[H]
    \caption{}
    \begin{algorithmic} 
            \item\textbf{Inputs:} $x_0\in\HH$, $y_0\in\mathcal{G}$
            \For{$n=0,\ldots$} 
                \State $\bar{x}_{n} =\prox_{\gamma_{1}f}(x_{n}-\gamma_{1}\sum_{j=1}^{r}L_{j}^{*}y_{j,n}-\gamma_{1}\nabla h(x_{n}))  $
                \State $\bar{y}_{i,n} =\prox_{\gamma_{i+1}g_{i}^{*}}(y_{i,n}+(1-\theta)\gamma_{i+1}L_{i}x_{n} $
                \State $\qquad \, +\theta\gamma_{i+1} L_{i}\bar{x}_{n} -\gamma_{i+1}\nabla l_{i}^{*}(y_{i,n}))\quad i=1,\ldots,r$
                \State $\tilde{x}_{n} =\bar{x}_{n}-x_{n},\tilde{y}_{i,n}=\bar{y}_{i,n}-y_{i,n}\quad i=1,\ldots,r  $
                \State $\tilde{z}_{n}=(\tilde{x}_{n},\tilde{\underline{y}}_{n})$
                \State $\displaystyle \alpha_{n} =\frac{\lambda_{n}\|\tilde{z}_{n}\|_{P}^{2}}{\|S^{-1/2}\left(H+M^{*}\right)\tilde{z}_{n}\|^{2}}  $ 
                \State $(x_{n+1},\underline{y}_{n+1}) =(x_{n},\underline{y}_{n})+\alpha_{n}S^{-1}(H+M^{*})\tilde{z}_{n}$
            \EndFor
    \end{algorithmic}
\end{algorithm}


All the special choices for $S$ discussed in section (\ref{sec:Saddle-point-problem})
can be applied here. We will consider one special case that reduces
to the algorithm introduced by Chen and Teboulle in \cite{chen1994proximal}. 


\subsubsection{Special Case: Chen-Teboulle 1994}
Take $\theta=1$, $\mu=1$, analogous to Algorithm \ref{Algorithm-3} we recover the following algorithm by
further setting $f\equiv0$, $h\equiv0$, $l=\iota_{\{0\}}$ and $\gamma_{3}=\gamma_{2}$: 
\begin{align*}
\bar{x}_{n} & =x_{n}-\gamma_{1}\sum_{i=1}^{2}L_{i}^{*}y_{i,n}\\
y_{1,n+1} & =\prox_{\gamma_{2}g_{1}^{*}}(y_{1,n}+\gamma_{2}L_{1}\bar{x}_{n})\\
y_{2,n+1} & =\prox_{\gamma_{2}g_{2}^{*}}(y_{1,n}+\gamma_{2}L_{2}\bar{x}_{n})\\
x_{n+1} & =x_{n}-\gamma_{1}\sum_{i=1}^{2}L_{i}^{*}y_{i,n+1}
\end{align*}
According to Proposition \ref{cor:coco-3}, it is convergent if
$\gamma_{1}^{-1}-\gamma_{2}\|\sum_{i=1}^{2}L_{i}^{*}L_{i}\|>0$.
Consider the problem: 
\begin{align*}
\minimize\: & f(x)+g(Ax)
\end{align*}
and the dual problem 
\begin{align*}
\minimize\: & f^{*}(-A^{*}y)+g^{*}(y).
\end{align*}
Apply the algorithm to the dual problem with
$g_{1}=f^{*}$, $g_{2}=g^{*}$ and $L_{1}=-A^{*}$, $L_{2}=I$ to obtain 
\begin{align*}
\bar{x}_{n} & =x_{n}+\gamma_{1}(Ay_{1,n}-y_{2,n})\\
y_{1,n+1} & =\prox_{\gamma_{2}f}(y_{1,n}-\gamma_{2}A^{*}\bar{x}_{n})\\
y_{2,n+1} & =\prox_{\gamma_{2}g}(y_{2,n}+\gamma_{2}\bar{x}_{n})\\
x_{n+1} & =x_{n}+\gamma_{1}(Ay_{1,n+1}-y_{2,n+1})
\end{align*}
where we require $\gamma_{1}^{-1}-\gamma_{2}\|AA^{*}+I\|>0$. If in addition $\gamma_{1}=\gamma_{2}$ then $\gamma^{2}\leq \frac{1}{\|A^{*}A+I\|}\}.$ Chen and Teboulle propose the same algorithm in \cite[Theorem 3.1]{chen1994proximal}
with a more conservative domain of convergence:
$\gamma\leq min\{\frac{1}{2},\frac{1}{2\|A\|}\}.$ \textcolor{red}{seems to me! they have weird parameters.}

\textcolor{red} {Add comment about nonzero off-diagonals}
